REINFOREST: Reinforcing Semantic Code Similarity for Cross-Lingual Code Search Models

This paper introduces a novel code-to-code search technique that enhances the performance of Large Language Models (LLMs) by including both static and dynamic features as well as utilizing both similar and dissimilar examples during training. We present the first-ever code search method that encodes dynamic runtime information during training without the need to execute either the corpus under search or the search query at inference time and the first code search technique that trains on both positive and negative reference samples. To validate the efficacy of our approach, we perform a set of studies demonstrating the capability of enhanced LLMs to perform cross-language code-to-code search. Our evaluation demonstrates that the effectiveness of our approach is consistent across various model architectures and programming languages. We outperform the state-of-the-art cross-language search tool by up to 44.7\%. Moreover, our ablation studies reveal that even a single positive and negative reference sample in the training process results in substantial performance improvements demonstrating both similar and dissimilar references are important parts of code search. Importantly, we show that enhanced well-crafted, fine-tuned models consistently outperform enhanced larger modern LLMs without fine tuning, even when enhancing the largest available LLMs highlighting the importance for open-sourced models. To ensure the reproducibility and extensibility of our research, we present an open-sourced implementation of our tool and training procedures called REINFOREST.

==> body/99.help_and_todo.tex <==
\section{Sketch of the paper}

\subsection{TODO}


\subsection{Help}
\begin{itemize}
    \item To write a code in one line, \linecode{public static void main (String args[])}
    \item To highlight something with a box, \\\highlight{This line needs to be highlighted}
    \item For writing any code with error \errorcode{statioc void main}
    \item To highlight a lesson learned, \lessons{lesson learned}
    \item To \textbf{repeat} an earlier research question \RQrepeat{1}{\rqa}
    \item To \textbf{answer} a RQ \RS{1}{The answer}.
    \item To leave comment for specific persons,
        \begin{itemize}
            \item \saikat{For assigning to Saikat}
            \item \anthony{For assigning to Anthony}
        \end{itemize}
\end{itemize}

==> tables/impact.tex <==
\begin{table*}[h]
\caption{\textbf{Impact of Positive and Negative samples. Max-p and Max-n stand for Maximum Positive samples and Maximum Negative samples, respectively.}}
\label{tab:impact}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cc||ccccccc||ccccccc}
\hlineB{2}
 &  &  & \multicolumn{7}{c||}{\textbf{Java}} & \multicolumn{7}{c}{\textbf{Python}} \bigstrut \\ \cline{4-17} 
\multirow{-2}{*}{\textbf{Model}} & \multirow{-2}{*}{\textbf{Max-p}} & \multirow{-2}{*}{\textbf{Max-N}} & \multicolumn{1}{c|}{\textbf{PR@1}} & \multicolumn{1}{c|}{\textbf{PR@2}} & \multicolumn{1}{c|}{\textbf{PR@3}} & \multicolumn{1}{c|}{\textbf{PR@4}} & \multicolumn{1}{c|}{\textbf{PR@5}} & \multicolumn{1}{c|}{\textbf{AFP}} & \textbf{ARG} & \multicolumn{1}{c|}{\textbf{PR@1}} & \multicolumn{1}{c|}{\textbf{PR@2}} & \multicolumn{1}{c|}{\textbf{PR@3}} & \multicolumn{1}{c|}{\textbf{PR@4}} & \multicolumn{1}{c|}{\textbf{PR@5}} & \multicolumn{1}{c|}{\textbf{AFP}} & \textbf{ARG} \bigstrut \\ \hlineB{2}
 & 5 & 5 & \multicolumn{1}{c|}{{ 86.47}} & \multicolumn{1}{c|}{{ 85.46}} & \multicolumn{1}{c|}{{ 84.77}} & \multicolumn{1}{c|}{{ 83.77}} & \multicolumn{1}{c|}{{ 82.62}} & \multicolumn{1}{c|}{{ 9.53}} & { 0.3857} & \multicolumn{1}{c|}{{ 94.05}} & \multicolumn{1}{c|}{{ 92.98}} & \multicolumn{1}{c|}{{ 92.01}} & \multicolumn{1}{c|}{{ 91.11}} & \multicolumn{1}{c|}{{ 90.37}} & \multicolumn{1}{c|}{{ 3.64}} & { 0.4051} \bigstrut \\ 
 & 5 & 0 & \multicolumn{1}{c|}{7.06} & \multicolumn{1}{c|}{7.06} & \multicolumn{1}{c|}{7.06} & \multicolumn{1}{c|}{7.06} & \multicolumn{1}{c|}{7.06} & \multicolumn{1}{c|}{215.26} & 0.0101 & \multicolumn{1}{c|}{5.29} & \multicolumn{1}{c|}{8.59} & \multicolumn{1}{c|}{7.19} & \multicolumn{1}{c|}{4.46} & \multicolumn{1}{c|}{7.08} & \multicolumn{1}{c|}{50.38} & 0.0476 \bigstrut \\ 
 & 0 & 5 & \multicolumn{1}{c|}{5.58} & \multicolumn{1}{c|}{4.24} & \multicolumn{1}{c|}{4.67} & \multicolumn{1}{c|}{4.82} & \multicolumn{1}{c|}{4.56} & \multicolumn{1}{c|}{150.72} & 0.0111 & \multicolumn{1}{c|}{8.84} & \multicolumn{1}{c|}{7.29} & \multicolumn{1}{c|}{5.75} & \multicolumn{1}{c|}{5.91} & \multicolumn{1}{c|}{5.4} & \multicolumn{1}{c|}{76.93} & -0.0109 \bigstrut \\ 
 & 1 & 1 & \multicolumn{1}{c|}{82.02} & \multicolumn{1}{c|}{81.6} & \multicolumn{1}{c|}{80.71} & \multicolumn{1}{c|}{79.94} & \multicolumn{1}{c|}{79.06} & \multicolumn{1}{c|}{9.82} & 0.3461 & \multicolumn{1}{c|}{93.41} & \multicolumn{1}{c|}{93} & \multicolumn{1}{c|}{92.36} & \multicolumn{1}{c|}{91.64} & \multicolumn{1}{c|}{91.04} & \multicolumn{1}{c|}{2.5} & 0.418 \bigstrut \\ 
\multirow{-7}{*}{\textbf{CodeBERT}} & 3 & 3 & \multicolumn{1}{c|}{83.5} & \multicolumn{1}{c|}{82.52} & \multicolumn{1}{c|}{81.58} & \multicolumn{1}{c|}{80.83} & \multicolumn{1}{c|}{79.88} & \multicolumn{1}{c|}{10.99} & 0.3612 & \multicolumn{1}{c|}{94.26} & \multicolumn{1}{c|}{93.13} & \multicolumn{1}{c|}{92.55} & \multicolumn{1}{c|}{91.78} & \multicolumn{1}{c|}{91.22} & \multicolumn{1}{c|}{2.45} & 0.3918 \bigstrut \\ \hlineB{2}
 & 5 & 5 & \multicolumn{1}{c|}{66.77} & \multicolumn{1}{c|}{65.85} & \multicolumn{1}{c|}{65.24} & \multicolumn{1}{c|}{64.58} & \multicolumn{1}{c|}{63.81} & \multicolumn{1}{c|}{10.6} & 0.3458 & \multicolumn{1}{c|}{87.88} & \multicolumn{1}{c|}{87.14} & \multicolumn{1}{c|}{86.45} & \multicolumn{1}{c|}{86.08} & \multicolumn{1}{c|}{85.45} & \multicolumn{1}{c|}{2.71} & 0.4037 \bigstrut \\ 
 & 5 & 0 & \multicolumn{1}{c|}{14.12} & \multicolumn{1}{c|}{15.85} & \multicolumn{1}{c|}{15.98} & \multicolumn{1}{c|}{15.98} & \multicolumn{1}{c|}{16.1} & \multicolumn{1}{c|}{76.73} & 0.087 & \multicolumn{1}{c|}{7.53} & \multicolumn{1}{c|}{9.2} & \multicolumn{1}{c|}{9.67} & \multicolumn{1}{c|}{9.92} & \multicolumn{1}{c|}{9.95} & \multicolumn{1}{c|}{39.85} & 0.1263 \bigstrut \\ 
 & 0 & 5 & \multicolumn{1}{c|}{5.46} & \multicolumn{1}{c|}{4.51} & \multicolumn{1}{c|}{4.69} & \multicolumn{1}{c|}{5.14} & \multicolumn{1}{c|}{5.61} & \multicolumn{1}{c|}{65.23} & 0.0342 & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{0.74} & \multicolumn{1}{c|}{1.59} & \multicolumn{1}{c|}{1.76} & \multicolumn{1}{c|}{1.98} & \multicolumn{1}{c|}{58.13} & 0.0407 \bigstrut \\ 
 & 1 & 1 & \multicolumn{1}{c|}{63.62} & \multicolumn{1}{c|}{62.08} & \multicolumn{1}{c|}{61.09} & \multicolumn{1}{c|}{60.06} & \multicolumn{1}{c|}{59.41} & \multicolumn{1}{c|}{15.98} & 0.326 & \multicolumn{1}{c|}{85.33} & \multicolumn{1}{c|}{84.59} & \multicolumn{1}{c|}{84.35} & \multicolumn{1}{c|}{83.44} & \multicolumn{1}{c|}{82.74} & \multicolumn{1}{c|}{2.46} & 0.3967 \bigstrut \\ 
\multirow{-7}{*}{\textbf{Ada}} & 3 & 3 & \multicolumn{1}{c|}{66.88} & \multicolumn{1}{c|}{64.84} & \multicolumn{1}{c|}{64.47} & \multicolumn{1}{c|}{63.34} & \multicolumn{1}{c|}{32.62} & \multicolumn{1}{c|}{12.21} & 0.3462 & \multicolumn{1}{c|}{87.29} & \multicolumn{1}{c|}{86.05} & \multicolumn{1}{c|}{85.25} & \multicolumn{1}{c|}{84.48} & \multicolumn{1}{c|}{83.95} & \multicolumn{1}{c|}{3.26} & 0.4024 \bigstrut \\ \hlineB{2}
 & 5 & 5 & \multicolumn{1}{c|}{62.79} & \multicolumn{1}{c|}{61.99} & \multicolumn{1}{c|}{61.48} & \multicolumn{1}{c|}{60.85} & \multicolumn{1}{c|}{60.25} & \multicolumn{1}{c|}{12.21} & 0.3327 & \multicolumn{1}{c|}{82.23} & \multicolumn{1}{c|}{80.23} & \multicolumn{1}{c|}{79.25} & \multicolumn{1}{c|}{78.21} & \multicolumn{1}{c|}{77.2} & \multicolumn{1}{c|}{3.32} & 0.3917 \bigstrut \\ 
 & 5 & 0 & \multicolumn{1}{c|}{20.59} & \multicolumn{1}{c|}{19.7} & \multicolumn{1}{c|}{17.94} & \multicolumn{1}{c|}{16.91} & \multicolumn{1}{c|}{16.22} & \multicolumn{1}{c|}{40.42} & 0.0951 & \multicolumn{1}{c|}{8.21} & \multicolumn{1}{c|}{8.25} & \multicolumn{1}{c|}{7.36} & \multicolumn{1}{c|}{7.38} & \multicolumn{1}{c|}{6.79} & \multicolumn{1}{c|}{39.12} & 0.0932 \bigstrut \\ 
 & 0 & 5 & \multicolumn{1}{c|}{3.98} & \multicolumn{1}{c|}{4.07} & \multicolumn{1}{c|}{4.41} & \multicolumn{1}{c|}{3.95} & \multicolumn{1}{c|}{4.26} & \multicolumn{1}{c|}{52.47} & 0.0331 & \multicolumn{1}{c|}{2.76} & \multicolumn{1}{c|}{3.19} & \multicolumn{1}{c|}{3.1} & \multicolumn{1}{c|}{3.89} & \multicolumn{1}{c|}{4.12} & \multicolumn{1}{c|}{49.13} & -0.0062 \bigstrut \\ 
 & 1 & 1 & \multicolumn{1}{c|}{57.27} & \multicolumn{1}{c|}{56.11} & \multicolumn{1}{c|}{55.21} & \multicolumn{1}{c|}{54.72} & \multicolumn{1}{c|}{53.97} & \multicolumn{1}{c|}{17.2} & 0.3115 & \multicolumn{1}{c|}{79.21} & \multicolumn{1}{c|}{77.95} & \multicolumn{1}{c|}{76.7} & \multicolumn{1}{c|}{75.67} & \multicolumn{1}{c|}{74.82} & \multicolumn{1}{c|}{3.003} & 0.384 \bigstrut \\ 
\multirow{-7}{*}{\textbf{Babbage}} & 3 & 3 & \multicolumn{1}{c|}{64.45} & \multicolumn{1}{c|}{62.88} & \multicolumn{1}{c|}{61.72} & \multicolumn{1}{c|}{60.79} & \multicolumn{1}{c|}{59.7} & \multicolumn{1}{c|}{11.84} & 0.3354 & \multicolumn{1}{c|}{80.95} & \multicolumn{1}{c|}{79.87} & \multicolumn{1}{c|}{78.81} & \multicolumn{1}{c|}{77.71} & \multicolumn{1}{c|}{76.9} & \multicolumn{1}{c|}{3.04} & 0.3916 \bigstrut \\ \hlineB{2}
 & 5 & 5 & \multicolumn{1}{c|}{73.18} & \multicolumn{1}{c|}{72.2} & \multicolumn{1}{c|}{71.18} & \multicolumn{1}{c|}{70.49} & \multicolumn{1}{c|}{69.91} & \multicolumn{1}{c|}{8.92} & 0.355 & \multicolumn{1}{c|}{88.44} & \multicolumn{1}{c|}{87.56} & \multicolumn{1}{c|}{86.78} & \multicolumn{1}{c|}{85.69} & \multicolumn{1}{c|}{84.93} & \multicolumn{1}{c|}{2.93} & 0.4112 \bigstrut \\ 
 & 5 & 0 & \multicolumn{1}{c|}{9.55} & \multicolumn{1}{c|}{13.74} & \multicolumn{1}{c|}{13.93} & \multicolumn{1}{c|}{13.72} & \multicolumn{1}{c|}{13.78} & \multicolumn{1}{c|}{44.02} & 0.11 & \multicolumn{1}{c|}{17.18} & \multicolumn{1}{c|}{16.65} & \multicolumn{1}{c|}{14.6} & \multicolumn{1}{c|}{12.76} & \multicolumn{1}{c|}{11.53} & \multicolumn{1}{c|}{49.28} & 0.0869 \bigstrut \\ 
 & 0 & 5 & \multicolumn{1}{c|}{5.52} & \multicolumn{1}{c|}{4.27} & \multicolumn{1}{c|}{3.26} & \multicolumn{1}{c|}{2.66} & \multicolumn{1}{c|}{3.78} & \multicolumn{1}{c|}{81.7674} & 0.0261 & \multicolumn{1}{c|}{1.32} & \multicolumn{1}{c|}{2.47} & \multicolumn{1}{c|}{3.26} & \multicolumn{1}{c|}{3.35} & \multicolumn{1}{c|}{3.31} & \multicolumn{1}{c|}{40.11} & 0.0051 \bigstrut \\ 
 & 1 & 1 & \multicolumn{1}{c|}{62.85} & \multicolumn{1}{c|}{62.76} & \multicolumn{1}{c|}{62.81} & \multicolumn{1}{c|}{62.3} & \multicolumn{1}{c|}{61.73} & \multicolumn{1}{c|}{12.02} & 0.3384 & \multicolumn{1}{c|}{82.48} & \multicolumn{1}{c|}{81.19} & \multicolumn{1}{c|}{80.1} & \multicolumn{1}{c|}{79.29} & \multicolumn{1}{c|}{78.57} & \multicolumn{1}{c|}{3.09} & 0.391 \bigstrut \\ 
\multirow{-7}{*}{\textbf{Curie}} & 3 & 3 & \multicolumn{1}{c|}{71.93} & \multicolumn{1}{c|}{70.5} & \multicolumn{1}{c|}{70.07} & \multicolumn{1}{c|}{69.36} & \multicolumn{1}{c|}{68.74} & \multicolumn{1}{c|}{11.26} & 0.3496 & \multicolumn{1}{c|}{87.5} & \multicolumn{1}{c|}{86.61} & \multicolumn{1}{c|}{86.18} & \multicolumn{1}{c|}{85.52} & \multicolumn{1}{c|}{84.89} & \multicolumn{1}{c|}{3.11} & 0.4059 \bigstrut \\ \hlineB{2}
 & 5 & 5 & \multicolumn{1}{c|}{68.07} & \multicolumn{1}{c|}{69.95} & \multicolumn{1}{c|}{67} & \multicolumn{1}{c|}{66.94} & \multicolumn{1}{c|}{66.53} & \multicolumn{1}{c|}{9.47} & 0.3543 & \multicolumn{1}{c|}{81.89} & \multicolumn{1}{c|}{81.1} & \multicolumn{1}{c|}{80.12} & \multicolumn{1}{c|}{79.52} & \multicolumn{1}{c|}{78.72} & \multicolumn{1}{c|}{3.59} & 0.3986 \bigstrut \\ 
 & 5 & 0 & \multicolumn{1}{c|}{3.5} & \multicolumn{1}{c|}{2.82} & \multicolumn{1}{c|}{3.72} & \multicolumn{1}{c|}{4.42} & \multicolumn{1}{c|}{5.08} & \multicolumn{1}{c|}{45.42} & 0.0468 & \multicolumn{1}{c|}{6.25} & \multicolumn{1}{c|}{6.25} & \multicolumn{1}{c|}{5.8} & \multicolumn{1}{c|}{5.68} & \multicolumn{1}{c|}{5.86} & \multicolumn{1}{c|}{49.86} & 0.0405 \bigstrut \\ 
 & 0 & 5 & \multicolumn{1}{c|}{3.98} & \multicolumn{1}{c|}{6.32} & \multicolumn{1}{c|}{4.79} & \multicolumn{1}{c|}{3.83} & \multicolumn{1}{c|}{3.65} & \multicolumn{1}{c|}{70.43} & 0.0011 & \multicolumn{1}{c|}{1.49} & \multicolumn{1}{c|}{0.87} & \multicolumn{1}{c|}{1.09} & \multicolumn{1}{c|}{0.84} & \multicolumn{1}{c|}{1.22} & \multicolumn{1}{c|}{46.26} & -0.0145 \bigstrut \\ 
 & 1 & 1 & \multicolumn{1}{c|}{41.13} & \multicolumn{1}{c|}{41.69} & \multicolumn{1}{c|}{42.02} & \multicolumn{1}{c|}{41.97} & \multicolumn{1}{c|}{41.73} & \multicolumn{1}{c|}{15.6} & 0.3218 & \multicolumn{1}{c|}{51.87} & \multicolumn{1}{c|}{50.83} & \multicolumn{1}{c|}{50.11} & \multicolumn{1}{c|}{50.05} & \multicolumn{1}{c|}{49.26} & \multicolumn{1}{c|}{6.61} & 0.3699 \bigstrut \\ 
\multirow{-7}{*}{\textbf{Davinci}} & 3 & 3 & \multicolumn{1}{c|}{62.91} & \multicolumn{1}{c|}{62.88} & \multicolumn{1}{c|}{62.51} & \multicolumn{1}{c|}{61.77} & \multicolumn{1}{c|}{61.19} & \multicolumn{1}{c|}{8.83} & 0.3452 & \multicolumn{1}{c|}{69.05} & \multicolumn{1}{c|}{68.75} & \multicolumn{1}{c|}{68.3} & \multicolumn{1}{c|}{67.92} & \multicolumn{1}{c|}{67.3} & \multicolumn{1}{c|}{5.22} & 0.3929 \bigstrut \\ \hlineB{2}
\end{tabular}%
}
\end{table*}

==> tables/main_result_java.tex <==
% \begin{table*}[t]
% % \small
% \centering
% \caption{\textbf{Java-Python Code Search}}
% \label{tab:java-python-main}
% \resizebox{\textwidth}{!}%
% {\begin{tabular}{c|c r|c|c|c c c c c|c|c}
% \hlineB{3}
% \multirow{2}{*}{\textbf{Model}} & \textbf{Sub-} & \textbf{Vector} &\multirow{2}{*}{\textbf{Trained}} & \textbf{Semantic} & \multicolumn{5}{c|}{\textbf{Mean Average Precision : MAP}} & \multirow{2}{*}{\textbf{APR@1}} & \multirow{2}{*}{\textbf{MRG}} \bigstrut[t]\bigstrut \\
% & \textbf{Model} & \textbf{Size} & &\textbf{Training}& \textbf{@1} & \textbf{@2} &\textbf{ @3} & \textbf{@4} &\textbf{ @5} & & \bigstrut[b]\bigstrut \\
% \hlineB{3}
% BM-25 & \multicolumn{4}{c|}{\multirow{3}{*}{No training   required}} & 15.14 & 13.56 & 12.25 & 11.59 & 11.17 & 48.93 & 0.1209 \bigstrut\bigstrut \\ \cline{1-1} \cline{6-12} 
% Token-Similarity~\cite{mathew2021cosal} & \multicolumn{4}{c|}{} & 59.76 & 57.95 & 56.08 & 54.79 & 53.73 & 20.71 & 0.2496 \bigstrut\bigstrut \\ \cline{1-1} \cline{6-12} 
% Tree-Similarity & \multicolumn{4}{c|}{} &  &  &  &  &  &  &  \bigstrut\bigstrut \\ \hlineB{3}
% \multirow{3}{*}{CodeBERT} & \multirow{3}{*}{-} & \multirow{3}{*}{768} & {\cross} & - & 10.50 & 10.06 & 9.73 & 9.70 & 9.42 & 48.95 & 0.0871 \bigstrut[t]\bigstrut \\  
%  &  & & {\tick} & \cross & 80.77 & 79.55 & 78.44 & 77.02 & 75.22 & 13.79 & 0.3407 \bigstrut \\ 
%  &  & & {\tick} & \tick & \textbf{86.47} & \textbf{85.46} &\textbf{ 84.77} & \textbf{83.77} & \textbf{82.62} & 9.53 & \textbf{0.3857} \bigstrut[b]\bigstrut \\ \hlineB{3}
% \multirow{13}{*}{Codex} & {\multirow{3}{*}{ada}} & {\multirow{3}{*}{1024}} & {\cross} & - & 34.07 & 32.99 & 32.23 & 31.94 & 31.55 & 19.69 & 0.1907 \bigstrut[t]\bigstrut \\ 
%  & {} & & {\tick} & \cross & 64.45 & 63.74 & 62.75 & 62.06 & 61.46 & 11.87 & 0.3442 \bigstrut \\ 
%  & {} & & {\tick} & \tick & 66.77 & 65.85 & 65.24 & 64.58 & 63.81 & 10.60 & 0.3458 \bigstrut[b]\bigstrut \\ \clineB{2-12}{2} 
%  & {\multirow{3}{*}{babbage}}& {\multirow{3}{*}{2048}} & {\cross} & - & 43.32 & 39.76 & 37.01 & 35.39 & 34.46 & 21.56 & 0.1833 \bigstrut[t]\bigstrut \\ 
%  & {} & &{\tick} & \cross & 58.69 & 58.13 & 57.62 & 57.21 & 56.94 & 16.80 & 0.3336 \bigstrut \\ 
%  & {} & &{\tick} & \tick & 62.79 & 61.99 & 61.48 & 60.85 & 60.25 & 12.21 & 0.3327 \bigstrut[b]\bigstrut \\ \clineB{2-12}{2} 
%  & {\multirow{3}{*}{curie}}& {\multirow{3}{*}{4096}} & {\cross} & - & 56.80 & 55.61 & 53.97 & 53.16 & 52.17 & 19.79 & 0.2507 \bigstrut[t]\bigstrut \\ 
%  & {} & &{\tick} & \cross & 69.97 & 68.52 & 67.83 & 67.42 & 66.73 & 10.99 & 0.3461 \bigstrut \\ 
%  & {} & &{\tick} & \tick & 73.18 & 72.20 & 71.18 & 70.49 & 69.91 & \textbf{8.92} & 0.3550 \bigstrut[b]\bigstrut \\ \clineB{2-12}{2} 
%  & {\multirow{3}{*}{davinci}}& {\multirow{3}{*}{12188}} & {\cross} & - & 44.93 & 42.11 & 40.91 & 39.84 & 38.99 & 11.91 & 0.2247 \bigstrut[t]\bigstrut \\ 
%  &  & &{\tick} & \cross & 56.69 & 56.58 & 56.66 & 56.47 & 56.15 & 15.43 & 0.3397 \bigstrut \\ 
%  &  & &{\tick} & \tick & 68.07 & 69.95 & 67.00 & 66.94 & 66.53 & 9.47 & 0.3543 \bigstrut[b]\bigstrut \\ \hlineB{3}
% \end{tabular}%
% }
% \end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[h]
\centering
\caption{\textbf{Detailed Results of Searching Python Code with Java Code as query}}
\label{tab:java_res}
% \resizebox{\textwidth}{!}
{%
\begin{tabular}{ccccc|ccccccc}
\hlineB{2}
\multicolumn{5}{c|}{\textbf{Settings}} & \multicolumn{7}{c}{\textbf{Metrics}} \bigstrut \\ \hlineB{2}
\multicolumn{1}{c|}{\textbf{Model}} & \multicolumn{1}{c|}{\textbf{Sub-Model}} & \multicolumn{1}{c|}{\textbf{Trained}} & \multicolumn{1}{c|}{\textbf{SSS}} & $\mathbf{\alpha}$ & \multicolumn{1}{c|}{\textbf{PR@1}} & \multicolumn{1}{c|}{\textbf{PR@2}} & \multicolumn{1}{c|}{\textbf{PR@3}} & \multicolumn{1}{c|}{\textbf{PR@4}} & \multicolumn{1}{c|}{\textbf{PR@5}} & \multicolumn{1}{c|}{\textbf{AFP}} & \textbf{ARG} \bigstrut \\ \hlineB{2}
\multicolumn{1}{c|}{BM25} & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}} & \multicolumn{1}{c|}{15.14} & \multicolumn{1}{c|}{13.56} & \multicolumn{1}{c|}{12.25} & \multicolumn{1}{c|}{11.59} & \multicolumn{1}{c|}{11.17} & \multicolumn{1}{c|}{48.93} & 0.1209 \bigstrut \\ \cline{1-1} \cline{6-12} 
\multicolumn{1}{c|}{Token-Subset (COSAL)} & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}} & \multicolumn{1}{c|}{59.76} & \multicolumn{1}{c|}{57.95} & \multicolumn{1}{c|}{56.08} & \multicolumn{1}{c|}{54.79} & \multicolumn{1}{c|}{53.73} & \multicolumn{1}{c|}{20.71} & 0.2496 \bigstrut \\ \cline{1-1} \cline{6-12} 
\multicolumn{1}{c|}{Tree-Similarity (stratified)} & \multicolumn{4}{c|}{\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}No-Training   required}} & \multicolumn{1}{c|}{53.33} & \multicolumn{1}{c|}{48.33} & \multicolumn{1}{c|}{47.04} & \multicolumn{1}{c|}{45.28} & \multicolumn{1}{c|}{43.11} & \multicolumn{1}{c|}{17.03} & 0.23336 \bigstrut \\ \hlineB{2}
\multicolumn{1}{c|}{} & \multicolumn{4}{c|}{CodeBERT  (stratified)} & \multicolumn{1}{c|}{29} & \multicolumn{1}{c|}{29} & \multicolumn{1}{c|}{29.17} & \multicolumn{1}{c|}{29} & \multicolumn{1}{c|}{29.5} & \multicolumn{1}{c|}{22.88} & 0.2947 \bigstrut \\ \cline{2-12} 
\multicolumn{1}{c|}{} & \multicolumn{4}{c|}{GraphCodeBERT    (stratified)} & \multicolumn{1}{c|}{13.5} & \multicolumn{1}{c|}{10.5} & \multicolumn{1}{c|}{10.67} & \multicolumn{1}{c|}{11.63} & \multicolumn{1}{c|}{11.9} & \multicolumn{1}{c|}{59.98} & 0.2814 \bigstrut \\ \cline{2-12} 
\multicolumn{1}{c|}{\multirow{-3}{*}{Single-Encoder   Models}} & \multicolumn{4}{c|}{UnixCoder  (stratified)} & \multicolumn{1}{c|}{61.5} & \multicolumn{1}{c|}{60} & \multicolumn{1}{c|}{62} & \multicolumn{1}{c|}{63} & \multicolumn{1}{c|}{63.4} & \multicolumn{1}{c|}{8.33} & 0.3559 \bigstrut \\ \hlineB{2}
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}-} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}N} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}-} & \cellcolor[HTML]{F8D8D8}- & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}10.5} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}10.06} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}9.73} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}9.7} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}9.42} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}48.95} & \cellcolor[HTML]{F8D8D8}0.0871 \bigstrut \\ \cline{2-12} 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{FCE5CD}-} & \multicolumn{1}{c|}{\cellcolor[HTML]{FCE5CD}Y} & \multicolumn{1}{c|}{\cellcolor[HTML]{FCE5CD}N} & \cellcolor[HTML]{FCE5CD}0 & \multicolumn{1}{c|}{\cellcolor[HTML]{FCE5CD}80.77} & \multicolumn{1}{c|}{\cellcolor[HTML]{FCE5CD}79.55} & \multicolumn{1}{c|}{\cellcolor[HTML]{FCE5CD}78.44} & \multicolumn{1}{c|}{\cellcolor[HTML]{FCE5CD}77.02} & \multicolumn{1}{c|}{\cellcolor[HTML]{FCE5CD}75.22} & \multicolumn{1}{c|}{\cellcolor[HTML]{FCE5CD}13.79} & \cellcolor[HTML]{FCE5CD}0.3407 \bigstrut \\ \cline{2-12} 
\multicolumn{1}{c|}{\multirow{-3}{*}{CodeBERT}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9EAD3}{\color[HTML]{00009B} \textbf{-}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9EAD3}{\color[HTML]{00009B} \textbf{Y}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9EAD3}{\color[HTML]{00009B} \textbf{Y}}} & \cellcolor[HTML]{D9EAD3}{\color[HTML]{00009B} \textbf{0.2}} & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}{\color[HTML]{00009B} \textbf{86.47}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}{\color[HTML]{00009B} \textbf{85.46}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}{\color[HTML]{00009B} \textbf{84.77}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}{\color[HTML]{00009B} \textbf{83.77}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}{\color[HTML]{00009B} \textbf{82.62}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}{\color[HTML]{00009B} \textbf{9.53}}} & \cellcolor[HTML]{00FF00}{\color[HTML]{00009B} \textbf{0.3857}} \bigstrut \\ \hlineB{2}
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}N} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}-} & \cellcolor[HTML]{F8D8D8}- & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}34.07} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}32.99} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}32.23} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}31.94} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}31.55} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}19.69} & \cellcolor[HTML]{F8D8D8}0.1907 \bigstrut \\ \cline{3-12} 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Y} & \multicolumn{1}{c|}{N} & 0 & \multicolumn{1}{c|}{64.45} & \multicolumn{1}{c|}{63.74} & \multicolumn{1}{c|}{62.75} & \multicolumn{1}{c|}{62.06} & \multicolumn{1}{c|}{61.46} & \multicolumn{1}{c|}{11.87} & 0.3442 \bigstrut \\ \cline{3-12} 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{-3}{*}{Ada}} & \multicolumn{1}{c|}{Y} & \multicolumn{1}{c|}{Y} & 0.2 & \multicolumn{1}{c|}{66.77} & \multicolumn{1}{c|}{65.85} & \multicolumn{1}{c|}{65.24} & \multicolumn{1}{c|}{64.58} & \multicolumn{1}{c|}{63.81} & \multicolumn{1}{c|}{10.6} & 0.3458 \bigstrut \\ \clineB{2-12}{2}
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}N} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}-} & \cellcolor[HTML]{F8D8D8}- & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}43.32} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}39.76} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}37.01} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}35.39} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}34.46} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}21.56} & \cellcolor[HTML]{F8D8D8}0.1833 \bigstrut \\ \cline{3-12} 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Y} & \multicolumn{1}{c|}{N} & 0 & \multicolumn{1}{c|}{58.69} & \multicolumn{1}{c|}{58.13} & \multicolumn{1}{c|}{57.62} & \multicolumn{1}{c|}{57.21} & \multicolumn{1}{c|}{56.94} & \multicolumn{1}{c|}{16.8} & 0.3336 \bigstrut \\ \cline{3-12} 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{-3}{*}{Babbage}} & \multicolumn{1}{c|}{Y} & \multicolumn{1}{c|}{Y} & 0.2 & \multicolumn{1}{c|}{62.79} & \multicolumn{1}{c|}{61.99} & \multicolumn{1}{c|}{61.48} & \multicolumn{1}{c|}{60.85} & \multicolumn{1}{c|}{60.25} & \multicolumn{1}{c|}{12.21} & 0.3327 \bigstrut \\ \clineB{2-12}{2}
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}N} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}-} & \cellcolor[HTML]{F8D8D8}- & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}56.8} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}55.61} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}53.97} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}53.16} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}52.17} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}19.79} & \cellcolor[HTML]{F8D8D8}0.2507 \bigstrut \\ \cline{3-12} 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Y} & \multicolumn{1}{c|}{N} & 0 & \multicolumn{1}{c|}{69.97} & \multicolumn{1}{c|}{68.52} & \multicolumn{1}{c|}{67.83} & \multicolumn{1}{c|}{67.42} & \multicolumn{1}{c|}{66.73} & \multicolumn{1}{c|}{10.99} & 0.3461 \bigstrut \\ \cline{3-12} 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{-3}{*}{Curie}} & \multicolumn{1}{c|}{Y} & \multicolumn{1}{c|}{Y} & 0.2 & \multicolumn{1}{c|}{73.18} & \multicolumn{1}{c|}{72.2} & \multicolumn{1}{c|}{71.18} & \multicolumn{1}{c|}{70.49} & \multicolumn{1}{c|}{69.91} & \multicolumn{1}{c|}{8.92} & 0.355 \bigstrut \\ \clineB{2-12}{2}
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}N} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}-} & \cellcolor[HTML]{F8D8D8}- & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}44.93} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}42.11} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}40.91} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}39.84} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}38.99} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}11.91} & \cellcolor[HTML]{F8D8D8}0.2247 \bigstrut \\ \cline{3-12} 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Y} & \multicolumn{1}{c|}{N} & 0 & \multicolumn{1}{c|}{56.69} & \multicolumn{1}{c|}{56.58} & \multicolumn{1}{c|}{56.66} & \multicolumn{1}{c|}{56.47} & \multicolumn{1}{c|}{56.15} & \multicolumn{1}{c|}{15.43} & 0.3397 \bigstrut \\ \cline{3-12} 
\multicolumn{1}{c|}{\multirow{-17}{*}{Codex}} & \multicolumn{1}{c|}{\multirow{-3}{*}{Davinci}} & \multicolumn{1}{c|}{Y} & \multicolumn{1}{c|}{Y} & 0.2 & \multicolumn{1}{c|}{68.07} & \multicolumn{1}{c|}{69.95} & \multicolumn{1}{c|}{67} & \multicolumn{1}{c|}{66.94} & \multicolumn{1}{c|}{66.53} & \multicolumn{1}{c|}{9.47} & 0.3543 \bigstrut \\ \hlineB{2}
\end{tabular}%
}
\end{table*}

==> tables/main_result_python.tex <==
% \begin{table*}[h]
% % \small
% \centering
% \caption{\textbf{Python to Java Code Search}}
% \label{tab:python-java-main}
% \resizebox{\textwidth}{!}%
% {\begin{tabular}{c|c rc|c|c c c c cc|c}
% \hlineB{2}B{3}
% \multirow{2}{*}{\textbf{Model}} & \textbf{Sub-} & \textbf{Vector} &\multirow{2}{*}{\textbf{Trained}} & \textbf{Semantic} & \multicolumn{5}{c|}{\textbf{Mean Average Precision : MAP}} & \multirow{2}{*}{\textbf{APR@1}} & \multirow{2}{*}{\textbf{MRG}} \bigstrut[t]\bigstrut \\
% & \textbf{Model} & \textbf{Size} & &\textbf{Training}& \textbf{@1} & \textbf{@2} &\textbf{ @3} & \textbf{@4} &\textbf{ @5} & & \bigstrut[b]\bigstrut \\
% \hlineB{2}B{3}
% BM-25 & \multicolumn{4}{c|}{\multirow{3}{*}{No training   required}} & 51.32 & 50.11 & 48.98 & 47.58 & 46.80 & 15.33 & 0.2649 \bigstrut\bigstrut \\ \cline{1-1} \cline{6-12} 
% Token-Similarity~\cite{mathew2021cosal} & \multicolumn{4}{c|}{} & 84.35 & 82.44 & 81.09 & 79.88 & 79.01 & 2.15 & 0.3073 \bigstrut\bigstrut \\ \cline{1-1} \cline{6-12} 
% Tree-Similarity & \multicolumn{4}{c|}{} &  &  &  &  &  &  &  \bigstrut\bigstrut \\ \hlineB{2}B{3}
% \multirow{3}{*}{CodeBERT} & \multirow{3}{*}{-} & \multirow{3}{*}{768} & {\cross} & - & 
%                 9.01	& 8.57  &	8.96	& 9.18 &	9.02&	48.58&	0.0875
% \bigstrut[t]\bigstrut \\  
%  &  & & {\tick} & \cross & 
%                 89.75&	87.48&	86.75&	85.44&	84.62&	3.42 &	0.3920
%  \bigstrut \\ 
%  &  & & {\tick} & \tick & 
%                  \textbf{94.05}&	\textbf{92.98}&	\textbf{92.01}&	\textbf{91.11}&	\textbf{90.37}&	3.64&	0.4051
%  \bigstrut[b]\bigstrut \\ \hlineB{2}B{3}
% \multirow{13}{*}{Codex} & {\multirow{3}{*}{ada}} & {\multirow{3}{*}{1024}} & {\cross} & - & 
%                  78.15&	76.19&	74.39&	73.14&	71.93&	3.91&	0.2378
% \bigstrut[t]\bigstrut \\ 
%  & {} & & {\tick} & \cross & 
%                 83.97&	83.69&	82.94&	81.64&	80.89&	3.57&	0.4040
% \bigstrut \\ 
%  & {} & & {\tick} & \tick & 
%                 87.88&	87.14&	86.45&	86.08&	85.45&	\textbf{2.71} &	0.4037
%  \bigstrut[b]\bigstrut \\ \clineB{2-12}{2} 
%  & {\multirow{3}{*}{babbage}}& {\multirow{3}{*}{2048}} & {\cross} & - & 
%                 76.36&	74.62&	72.97&	71.56&	70.36&	3.68&	0.2395
%  \bigstrut[t]\bigstrut \\ 
%  & {} & &{\tick} & \cross & 
%                 80.31&	78.78&	78.3&	77.56&	76.99&	3.88&	0.3986
% \bigstrut \\ 
%  & {} & &{\tick} & \tick & 
%                  82.23&	80.23&	79.25&	78.21&	77.2&	3.32&	0.3917
% \bigstrut[b]\bigstrut \\ \clineB{2-12}{2} 
%  & {\multirow{3}{*}{curie}}& {\multirow{3}{*}{4096}} & {\cross} & - & 
%                 75.89&	74.38&	73.44&	71.9&	70.82&	11.44&	0.2300
% \bigstrut[t]\bigstrut \\ 
%  & {} & &{\tick} & \cross & 
%                 82.14&	81.85&	81.29&	80.72&	80.19&	3.29&	\textbf{0.4081}
% \bigstrut \\ 
%  & {} & &{\tick} & \tick & 
%                 88.44&	87.56&	86.78&	85.69&	84.93&	2.93&	0.4112
% \bigstrut[b]\bigstrut \\ \clineB{2-12}{2} 
%  & {\multirow{3}{*}{davinci}}& {\multirow{3}{*}{12188}} & {\cross} & - & 
%                 45.2&	44.66&	43.13&	42.09&	41.05&	10.03&	0.2082
% \bigstrut[t]\bigstrut \\ 
%  &  & &{\tick} & \cross & 
%                 68.11&	68.26&	67.90&	67.28&	66.96&	4.85&	0.3799
% \bigstrut \\ 
%  &  & &{\tick} & \tick & 
%                81.89&	81.10&	80.12&	79.52&	78.72&	3.59&	0.3986
% \bigstrut[b]\bigstrut \\ \hlineB{2}B{3}
% \end{tabular}%
% }
% \end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[h]
\centering
\caption{\textbf{Detailed Results of Searching Java Code with Python Code as query}}
\label{tab:python_res}
% \resizebox{\textwidth}{!}
{%
\begin{tabular}{ccccc|ccccccc}
\hlineB{2}
\multicolumn{5}{c|}{\textbf{Settings}} & \multicolumn{7}{c}{\textbf{Metrics}} \bigstrut \\ \hlineB{2}
\multicolumn{1}{c|}{\textbf{Model}} & \multicolumn{1}{c|}{\textbf{Sub-Model}} & \multicolumn{1}{c|}{\textbf{Trained}} & \multicolumn{1}{c|}{\textbf{SSS}} & $\alpha$ & \multicolumn{1}{c|}{\textbf{PR@1}} & \multicolumn{1}{c|}{\textbf{PR@2}} & \multicolumn{1}{c|}{\textbf{PR@3}} & \multicolumn{1}{c|}{\textbf{PR@4}} & \multicolumn{1}{c|}{\textbf{PR@5}} & \multicolumn{1}{c|}{\textbf{AFP}} & \textbf{ARG} \bigstrut \\ \hlineB{2}
\multicolumn{1}{c|}{BM25} & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}} & \multicolumn{1}{c|}{51.32} & \multicolumn{1}{c|}{50.11} & \multicolumn{1}{c|}{48.98} & \multicolumn{1}{c|}{47.58} & \multicolumn{1}{c|}{46.8} & \multicolumn{1}{c|}{15.33} & 0.2649 \bigstrut \\ \cline{1-1} \cline{6-12} 
\multicolumn{1}{c|}{Token-Subset (COSAL)} & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}} & \multicolumn{1}{c|}{84.35} & \multicolumn{1}{c|}{82.44} & \multicolumn{1}{c|}{81.09} & \multicolumn{1}{c|}{79.88} & \multicolumn{1}{c|}{79.01} & \multicolumn{1}{c|}{2.15} & 0.3073 \bigstrut \\ \cline{1-1} \cline{6-12} 
\multicolumn{1}{c|}{Tree-Similarity  (stratified)} & \multicolumn{4}{c|}{\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}No-Training   required}} & \multicolumn{1}{c|}{74.29} & \multicolumn{1}{c|}{71.35} & \multicolumn{1}{c|}{68.56} & \multicolumn{1}{c|}{66.05} & \multicolumn{1}{c|}{65.35} & \multicolumn{1}{c|}{8.56} & 0.2456 \bigstrut \\ \hlineB{2}
\multicolumn{1}{c|}{} & \multicolumn{4}{c|}{CodeBERT  (stratified)} & \multicolumn{1}{c|}{15.5} & \multicolumn{1}{c|}{16.75} & \multicolumn{1}{c|}{17.83} & \multicolumn{1}{c|}{18.38} & \multicolumn{1}{c|}{18.1} & \multicolumn{1}{c|}{130.33} & 0.2248 \bigstrut \\ \cline{2-12} 
\multicolumn{1}{c|}{} & \multicolumn{4}{c|}{GraphCodeBERT    (stratified)} & \multicolumn{1}{c|}{20.5} & \multicolumn{1}{c|}{21} & \multicolumn{1}{c|}{21.83} & \multicolumn{1}{c|}{22.25} & \multicolumn{1}{c|}{22.7} & \multicolumn{1}{c|}{142.85} & 0.2099 \bigstrut \\ \cline{2-12} 
\multicolumn{1}{c|}{\multirow{-3}{*}{Single-Encoder   Models}} & \multicolumn{4}{c|}{UnixCoder  (stratified)} & \multicolumn{1}{c|}{25} & \multicolumn{1}{c|}{25.25} & \multicolumn{1}{c|}{25.17} & \multicolumn{1}{c|}{25.88} & \multicolumn{1}{c|}{25.9} & \multicolumn{1}{c|}{57.5} & 0.3553 \bigstrut \\ \hlineB{2}
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}-} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}N} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}-} & \cellcolor[HTML]{F8D8D8}- & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}9.01} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}8.57} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}8.96} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}9.18} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}9.02} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}48.58} & \cellcolor[HTML]{F8D8D8}0.0875 \bigstrut \\ \cline{2-12} 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{FCE5CD}-} & \multicolumn{1}{c|}{\cellcolor[HTML]{FCE5CD}Y} & \multicolumn{1}{c|}{\cellcolor[HTML]{FCE5CD}N} & \cellcolor[HTML]{FCE5CD}0 & \multicolumn{1}{c|}{\cellcolor[HTML]{FCE5CD}89.75} & \multicolumn{1}{c|}{\cellcolor[HTML]{FCE5CD}87.48} & \multicolumn{1}{c|}{\cellcolor[HTML]{FCE5CD}86.75} & \multicolumn{1}{c|}{\cellcolor[HTML]{FCE5CD}85.44} & \multicolumn{1}{c|}{\cellcolor[HTML]{FCE5CD}84.62} & \multicolumn{1}{c|}{\cellcolor[HTML]{FCE5CD}3.424} & \cellcolor[HTML]{FCE5CD}0.392 \bigstrut \\ \cline{2-12} 
\multicolumn{1}{c|}{\multirow{-3}{*}{CodeBERT }} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9EAD3}{\color[HTML]{00009B} \textbf{-}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9EAD3}{\color[HTML]{00009B} \textbf{Y}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9EAD3}{\color[HTML]{00009B} \textbf{Y}}} & \cellcolor[HTML]{D9EAD3}{\color[HTML]{00009B} \textbf{0.2}} & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}{\color[HTML]{00009B} \textbf{94.05}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}{\color[HTML]{00009B} \textbf{92.98}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}{\color[HTML]{00009B} \textbf{92.01}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}{\color[HTML]{00009B} \textbf{91.11}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}{\color[HTML]{00009B} \textbf{90.37}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}{\color[HTML]{00009B} \textbf{3.64}}} & \cellcolor[HTML]{00FF00}{\color[HTML]{00009B} \textbf{0.4051}} \bigstrut \\ \hlineB{2}
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}N} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}-} & \cellcolor[HTML]{F8D8D8}- & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}78.15} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}76.19} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}74.39} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}73.14} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}71.93} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}3.91} & \cellcolor[HTML]{F8D8D8}0.2378 \bigstrut \\ \cline{3-12} 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Y} & \multicolumn{1}{c|}{N} & 0 & \multicolumn{1}{c|}{83.97} & \multicolumn{1}{c|}{83.69} & \multicolumn{1}{c|}{82.94} & \multicolumn{1}{c|}{81.64} & \multicolumn{1}{c|}{80.89} & \multicolumn{1}{c|}{3.57} & 0.404 \bigstrut \\ \cline{3-12} 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{-3}{*}{Ada}} & \multicolumn{1}{c|}{Y} & \multicolumn{1}{c|}{Y} & 0.2 & \multicolumn{1}{c|}{87.88} & \multicolumn{1}{c|}{87.14} & \multicolumn{1}{c|}{86.45} & \multicolumn{1}{c|}{86.08} & \multicolumn{1}{c|}{85.45} & \multicolumn{1}{c|}{2.71} & 0.4037 \bigstrut \\ \clineB{2-12}{2} 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}N} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}-} & \cellcolor[HTML]{F8D8D8}- & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}76.36} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}74.62} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}72.97} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}71.56} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}70.36} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}3.68} & \cellcolor[HTML]{F8D8D8}0.2395 \bigstrut \\ \cline{3-12} 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Y} & \multicolumn{1}{c|}{N} & 0 & \multicolumn{1}{c|}{80.31} & \multicolumn{1}{c|}{78.78} & \multicolumn{1}{c|}{78.3} & \multicolumn{1}{c|}{77.56} & \multicolumn{1}{c|}{76.99} & \multicolumn{1}{c|}{3.88} & 0.3986 \bigstrut \\ \cline{3-12} 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{-3}{*}{Babbage}} & \multicolumn{1}{c|}{Y} & \multicolumn{1}{c|}{Y} & 0.2 & \multicolumn{1}{c|}{82.23} & \multicolumn{1}{c|}{80.23} & \multicolumn{1}{c|}{79.25} & \multicolumn{1}{c|}{78.21} & \multicolumn{1}{c|}{77.2} & \multicolumn{1}{c|}{3.32} & 0.3917 \bigstrut \\ \clineB{2-12}{2} 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}N} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}-} & \cellcolor[HTML]{F8D8D8}- & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}75.89} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}74.38} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}73.44} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}71.9} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}70.82} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}11.44} & \cellcolor[HTML]{F8D8D8}0.23 \bigstrut \\ \cline{3-12} 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Y} & \multicolumn{1}{c|}{N} & 0 & \multicolumn{1}{c|}{82.14} & \multicolumn{1}{c|}{81.85} & \multicolumn{1}{c|}{81.29} & \multicolumn{1}{c|}{80.72} & \multicolumn{1}{c|}{80.19} & \multicolumn{1}{c|}{3.29} & 0.4081 \bigstrut \\ \cline{3-12} 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{-3}{*}{Curie}} & \multicolumn{1}{c|}{Y} & \multicolumn{1}{c|}{Y} & 0.2 & \multicolumn{1}{c|}{88.44} & \multicolumn{1}{c|}{87.56} & \multicolumn{1}{c|}{86.78} & \multicolumn{1}{c|}{85.69} & \multicolumn{1}{c|}{84.93} & \multicolumn{1}{c|}{2.93} & 0.4112 \bigstrut \\ \clineB{2-12}{2} 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}N} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}-} & \cellcolor[HTML]{F8D8D8}- & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}45.2} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}44.66} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}43.13} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}42.09} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}41.05} & \multicolumn{1}{c|}{\cellcolor[HTML]{F8D8D8}10.03} & \cellcolor[HTML]{F8D8D8}0.2082 \bigstrut \\ \cline{3-12} 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Y} & \multicolumn{1}{c|}{N} & 0 & \multicolumn{1}{c|}{68.11} & \multicolumn{1}{c|}{68.26} & \multicolumn{1}{c|}{67.9} & \multicolumn{1}{c|}{67.28} & \multicolumn{1}{c|}{66.96} & \multicolumn{1}{c|}{4.85} & 0.3799 \bigstrut \\ \cline{3-12} 
\multicolumn{1}{c|}{\multirow{-12}{*}{Codex}} & \multicolumn{1}{c|}{\multirow{-3}{*}{Davinci}} & \multicolumn{1}{c|}{Y} & \multicolumn{1}{c|}{Y} & 0.2 & \multicolumn{1}{c|}{81.89} & \multicolumn{1}{c|}{81.1} & \multicolumn{1}{c|}{80.12} & \multicolumn{1}{c|}{79.52} & \multicolumn{1}{c|}{78.72} & \multicolumn{1}{c|}{3.59} & 0.3986 \bigstrut \\ \hlineB{2}
\end{tabular}%
}
\end{table*}

==> todo.tex <==
1. Add acknowledgement section. 


% \section*{Response to the meta-reviews from ASE}


% % \subsection*{Required TODO}
% {\it The reviewers all agree that the work is promising but there are several weak points that need to be addressed before final acceptance. The weak points include:}

% {\color{blue} We thank the reviewers for their valuable comments and feedback on our work. In this version, we addressed the required TODOs mentioned in the meta-review, as per ASE guidelines. We annotated this manuscript highlighting the changes in \blue{blue}. 
% % Note that, in this revision, we added line number and page number for quick referencing between review comment and actual change. In the camera ready version, we will abide by the formatting requirement of ASE. 
% We are working on addressing other comments in the detailed reviews, which we hope to submit with the camera-ready version of the paper.}
% %Our response to the comments in meta review are as follow.}
% %We sincerely hope this version of the paper is acceptable.}

% \begin{enumerate}
%     \item {\it Clarify the modalities claim. Currently, the authors refer to three modalities, but the context and the lines can be considered as the same modality, i.e., both are represented in code.}
    
%     {\color{blue}
%     % - \Cref{sec:tool} - 224
%     - Thanks for this comment. We do acknowledge that code to be edited is essentially a substring of the context presented. However, by extracting such code, we provide MODIT with additional information about the change location. Thus, we prefer to consider ``code needs to be edited" as a separate mode of information (i.e., modality) indicating change location than code context. We clarified this point in Section-I, at the beginning of Section-III, and the experimental design of RQ2 (Section-V).
%     }
    
%     \item {\it Clarify or or remove claims of significance. When the paper claims that MODIT 'generates significantly more correct patches than models trained from scratch', the paper should back up that claim.}
    
%     {\color{blue} 
%     % - \Cref{sec:results} - RQ1 result(470-474), RQ2 lessons 1 (627-631).
%     - Thanks for this comment; We apologize for the misunderstanding. Our improvement comes from two design choices: 
    
%     \begin{itemize}
%         \item RQ1: pre-training vs. training from scratch: Our empirical results show that results are {\em significantly} improved when we use a pre-trained model, in contrast to a model trained from scratch for code editing (see Table-II). We have clarified this point in RQ1.
%     % ~\rayb{give line numbers}
%     \item RQ2: multi-modality: We have reworded our claim (see lessons learned), saying each of the modalities contribute to some extent to improve the overall performance (Section-V). 
%     % ~\rayb{give line numbers}
%     \end{itemize}
    
    
    
    
%     .
%     }
    
%     \item {\it Re-write the related work. Related work section has too many links, and does not really compare and contrast previous work with this paper. The authors should remove some citations and also have a more in-depth discussion of the related work. Every related work should be presented in relation to the work of this paper.}
    
%     {
%     \color{blue}
%     - Thanks for the suggestion. We have reorganized the related work putting more emphasis on the insights from existing works in the literature. 
%     }
    
% \end{enumerate}


% % \subsection*{Additional Changes}
% % \begin{itemize}
% %     \item \textbf{{\color{red}[Must - Writing]} R1.} The writeup for RQ2 could be more clear. Table III is difficult to parse. 
    
% %     {\color{blue}- RQ2 (555-563).}
    
% %     \item \textbf{{\color{red}[Must - Writing]} R2.} One of the novelty of the proposed approach is to involve the commit messages. But as we know, developers usually write commit messages after the code editing. Writing commit messages as guidance for code editing may cost developers’ time and efforts. Also, it cannot be guaranteed that the guidance is exactly clear before the code editing. Such concern may hinder the practicability of the proposed approach.
    
% %     {\color{blue} - \Cref{sec:threats} (843-853).}
    
% %     \item \textbf{{\color{orange}[Maybe - Exp]} R2.} In Tufano et al.’s work [8], different beam sizes are experimented. Since the beam search size can impact the computed accuracy, it would be better to test the results with different beam search sizes.
% %     \item \textbf{{\color{orange}[Maybe - Exp]} R2.} In Section VI-A, reporting the location prediction accuracy and comparing with the baseline approaches can make the answer more convincing and comprehensive.
    
% %     \item \textbf{{\color{orange}[Maybe - Exp]} R3.} The paper does not provide results in terms of syntax correctness of the code editing suggestions. Approaches like CODIT can guarantee syntax correctness of the suggestions, while the proposed approach does not. For this reason, it would be important to provide empirical evidence that MODIT can actually suggests syntactically correct code in most cases. Additionally, while I agree that the top-1 suggestion is the most interesting one and recommendation system should focus on the top-k suggestions the authors should provide an idea of how are the results outside the top-1.
    
% % \end{itemize}
% % % \pagebreak
